HumanEvo: An Evolution-aware Benchmark for More Realistic Evaluation of Repository-level Code Generation

To evaluate the repository-level code generation capabilities of Large Language Models (LLMs) in complex real-world software development scenarios, many evaluation methods have been developed. These methods typically leverage contextual code from the latest version of a project to assist LLMs in accurately generating the desired function. However, such evaluation methods fail to consider the dynamic evolution of software projects over time, which we refer to as evolution-ignored settings. This in turn results in inaccurate evaluation of LLMs' performance. In this paper, we conduct an empirical study to deeply understand LLMs' code generation performance within settings that reflect the evolution nature of software development. To achieve this, we first construct an evolution-aware repository-level code generation dataset, namely HumanEvo, equipped with an automated execution-based evaluation tool. Second, we manually categorize HumanEvo according to dependency levels to more comprehensively analyze the model's performance in generating functions with different dependency levels. Third, we conduct extensive experiments on HumanEvo with seven representative and diverse LLMs to verify the effectiveness of the proposed benchmark. We obtain several important findings through our experimental study. For example, we find that previous evolution-ignored evaluation methods result in inflated performance of LLMs, with performance overestimations ranging from 10.0% to 61.1% under different context acquisition methods, compared to the evolution-aware evaluation approach. Based on the findings, we give actionable suggestions for more realistic evaluation of LLMs on code generation. We also build a shared evolution-aware code generation toolbox to facilitate future research.

==> sections/1_Introduction.tex <==
\section{Introduction}
%%%背景
In recent years, LLMs have rapidly advanced and achieved remarkable accomplishments in the field of code generation. Many large language models for code, such as Codellama\cite{codellama}, StarCoder\cite{starcoder}, DeepSeek-Coder\cite{deepseek},  have illuminated the path toward automated code generation. Consequently, many of these large models are being employed to empower programming assistants, like DeepMind’s AlphaCode, Github Copilot, and are playing vital role in practical software development.

%

%%%现有工作：引入repo-level的重要性

With the emergence of an increasing number of LLMs, there has been a corresponding surge in the development of benchmarks aimed at evaluating the performance of these models in code generation tasks.  Prominent benchmarks such as HumanEval\cite{humaneval}, MBPP\cite{MBPP} and DS-1000\cite{DS1000} are widely utilized for assessing the capabilities of code LLMs.  However, many of these benchmarks primarily consist of standalnoe function task instances, which may not fully capture the complexities encountered in practical development scenarios. In real-world software development, functions typically exhibit numerous inter-dependencies with other functions. When programmers write a particular function, they need to refer to existing code files in the repository and thoroughly understand the mutual dependencies among the code components to accurately complete the programming task. A defining characteristic of function instances in pragmatic development is their tendency to have multiple dependencies. Unfortunately, benchmarks like HumanEval, MBPP and DS-1000 overlook this aspect, failing to adequately reflect the intricacies of functions encountered in real-world development environments.

%
%%%repo-level现有工作以及其缺点
%每个task instance都会对应着一个自然语言描述，大语言模型的任务就是根据这些自然语言描述以及附上的一些项目context生成目标代码。项目context的作用是帮助LLM尽可能了解项目中复杂的依赖关系和基本情况，一般通过相似性检索和静态分析来获得这些项目context。

Fortunately, several repository-level code generation initiatives have emerged to better simulate real-world development scenarios, such as CoderEval\cite{codereval}, RepoBench\cite{repobench}, and DevEval\cite{deveval}. These endeavors involve selecting task instances from existing code repositories to construct benchmark datasets, each of which corresponds to a natural language description. The the task of the large language models is to generate target code based on these natural language descriptions and the accompanying project context. The purpose of the project context is to assist the LLM in understanding the complex dependencies as much as possible, typically obtained through similarity retrieval and static analysis.



%repo-level benmark 的缺点 引入主题

However, previous efforts treat the latest version of the repository as the sole source of context, overlooking the dynamic evolution of projects over time.
% context source contains too much "extra" information. 
Specifically, modern software development is an incremental development process, meaning that projects evolve through multiple versions over time. When programmers develop based on version 1 of a project, the only project context they should refer to is all the code corresponding to version 1 of the repository, which is indisputable. Existing repository-level code generation benchmarks overlook the evolving nature of software projects by providing the latest codebase version as the context source. We term this the "evolving-ignored" situation. Actually, each function should have a different context corresponding to the project state at the time of its development. "Evolving-ignored" stiuation poses two main risks: \textbf{On one hand}, as in Figure \ref{figure1}, an excessive amount of "extra" project context may lead to unfairness in the performance of LLMs in previous benchmarks. \textbf{On the other hand}, as in Figure \ref{figure2}, with the project evolving, some useful context may have been updated or removed. Consequently, while the context provided by the latest version of the project miss these beneficial context, resulting in a disparity between contexts.




%whose natural summary are then used to prompt large language models (LLMs) to generate corresponding functions. (However, ...issues, ...)However, 




% In this paper, we propose CoderEval2, a xxx benchmark that .... Specificially, ....


% 引出自己的工作
Therefore, in this paper, we propose a novel code generation benchmark: Evolving-aware Repository-level code generation benchmark (CoderEval2), which better simulate real-world development processes and reflect the evolving nature of projects over time. Specifically, we drew inspiration from software development based on GitHub. When programmers complete and verify a portion of code, they update it to GitHub via commits. Hence, when programmers write a particular piece of code, the project context they can reference is the entire project before the programmer's commit action. Based on this, in order to provide the LLM with a better understanding of the current status of the project, we first rollback the entire project repository to the state before the target code was committed. Such an operation ensures that the context we provide precisely encompasses all the context available to the programmer when completing this function, neither including additional code introduced by subsequent version changes nor omitting code that may have been updated or deleted due to version changes. CoderEval2 consist of 400 programming problems, 200 for Python and 200 for Java, all of which are sampled from real-world high-quality projects. 

% To enhance the representativeness of CoderEval2, we followed five steps to obtain high-quality task instances from real-world GitHub projects. 
% First, we selected popular and highly-starred open-source Python and Java repositories. We focused on popular repositories because they are typically better maintained, have clear contributor guidelines, and boast better test coverage.
% Second, we collected a significant number of pull requests (PRs) from these repositories. In real-world GitHub-based projects, the incremental development process is often based on PRs. Developers complete a feature and then request that the newly added code be merged into the project repository by initiating a PR. Each PR is associated with a codebase, representing the state of the repository before the PR was merged. Our objective is for LLMs to generate single functions added in PRs based on the PR-associated codebase and corresponding natural language descriptions, thus simulating programming activities in actual software development.
% Third, we conducted an initial screening of the PRs obtained in the second step. We required each PR to add a new function because project maintenance is also based on PRs. Some PRs may not add new functions but only perform code edits or bug fixes, which are less relevant to our task. Additionally, we required each PR to make certain modifications to the test files in the repository, which typically implies that developers contributed tests to check if the added code meets requirements or contains bugs.
% Fourth, we completed the final screening through execution-based testing. For each candidate task, we applied the test content from the PR and recorded the associated test results before and after applying the PR's other content. We filtered out task instances without at least one test where its status changes from a fail to pass (referred to as fail-to-pass test). We also filtered out instances that result in installation or runtime errors.
% Fifth, after completing the above four steps, we had constructed the data portion of CoderEval2. However, due to various issues with comments in actual projects (e.g., overly long or short comments, or even the absence of comments), we recruited six experienced engineers to rewrite the docstring for each task instance. To enrich the diversity of our benchmark dataset, we generated two styles of comments for each function: detailed comments (mimicking model-generated comments, providing detailed descriptions of function functionality, and annotating each parameter and return value in detail) and brief comments (mimicking human-generated comments, providing only a simple introduction to the function's functionality).

To more accurately assess the correctness of code generated by large models, we adopt an execution-based evaluation approach. Due to potential dependencies on different third-party libraries or testing platforms at various project stages, we meticulously prepare a test suite for each version of every project. Encompassing multiple state-of-the-art LLMs such as the Codellama series, Deepseek-Coder series\cite{deepseek}, GPT-4\cite{gpt4}, and ChatGPT, we conduct extensive experiments on CoderEval2. Experimental results emphasize the importance of evolving-awareness, showcasing how LLMs gradually deviate from reality in evolving-ignored situations.

% First, we elucidate the differing performance of LLMs in both the evolving-ignored and evolving-aware scenarios. Subsequently, we partitioned CoderEval2's dataset into three parts based on dependency levels: standalone, intra-class, inter-class, thoroughly assessing and analyzing LLM performance across these three dependency levels. Lastly, we evaluated LLM performance under the two aforementioned natural language description prompts, revealing the true effectiveness of these models in real-world development scenarios. This comprehensive evaluation highlights the ongoing journey towards seamlessly integrating LLMs into practical development contexts, thereby providing valuable insights for the future advancement of code-centric large models.







In summary, our main contributions can be summarized as follows:

\begin{itemize}
    \item We point out the  common flaw of previous repository-level code generation benchmarks, analyze their potential impacts, and highlight the significance of evolving awareness. 
    \item We introduce a novel benchmark: the evolving-aware repository-level code generation benchmark, which addresses the issue of evolving ignorance present in previous repository-level code generation benchmarks. 
    \item Through extensive experimentation, we substantiate the dangers posed by the evolving-ignored situation and provide a better simulation of real-world development scenarios for repository-level code generation tasks.
\end{itemize}



% \begin{itemize}

%     \item  We identify common flaws in existing repository-level code generation benchmarks and demonstrate the disparity between the real performance of large models when future code is and isn't considered.
%     \item We introduced CoderEval2, a novel evolving-aware code generation benchmark. CoderEval2 addresses the evolving-ignored issue in existing benchmarks within the repository-level code generation domain concerning context aspects.
%     \item We provide a diverse evaluation strategy for different kinds of NL descripions, in which "model-like" and "human-like" styles., along with a thorough test suite comprises both integration and unit tests to ensure comprehensive testing coverage.
%     \item We conducted evaluations on multiple mainstream LLMs, better revealing their performance in real-world development scenarios. This highlights the significant progress needed before LLMs can be seamlessly applied in practical development contexts, thereby providing valuable guidance for the future development of code-centric large models.
    
% \end{itemize}


%Dynamic Context Inclusion: EvoEval dynamically includes only the context available at the time of code generation, avoiding the inclusion of future code snippets.

%Incremental Development Simulation: Our benchmark simulates incremental development scenarios, where the repository's context evolves over time, mirroring real-world software development practices.

%Versioned Test Suites: EvoEval prepares versioned test suites for each project version, ensuring comprehensive testing coverage tailored to the specific dependencies of each iteration.

%Integration and Unit Testing: The test suite includes both integration and unit tests to thoroughly evaluate the generated code's correctness and compatibility with the project's dependencies.

%Evaluation of Large Models: EvoEval evaluates multiple state-of-the-art large models, providing insights into their performance under evolving context scenarios.








% To more accurately assess the correctness of code generated by large models, we employ an execution-based evaluation approach. Given that projects may rely on different third-party libraries or testing platforms at different times, we meticulously prepare a test suite for each version of every project. Some prior works have also utilized execution-based methods to ensure that the functions generated by LLMs can satisfy the complex dependencies present in real projects. They typically generate multiple test cases for each function to evaluate the generated code, focusing solely on individual functions without fully considering the integration testing necessary for the project's complex dependencies. Therefore, relying solely on test cases for evaluation is inadequate when it comes to project-level testing. Hence, our test suite comprises both integration and unit tests to ensure comprehensive testing coverage.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/Figure1.pdf}
  \caption{Evolving-ignored situation one: too much "extra" context}
  \label{figure1}
\end{figure}

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/Figure2.pdf}
  \caption{Evolving-ignored situation one: missing too much context}
  \label{figure2}
\end{figure}

==> sections/2_Background.tex <==
\section{Background}
%介绍code LLM
% 介绍可以用于代码生成的benchmark
% 介绍repo-level相关的技术工作。
The emergence of generative large language models sheds light on automated code generation, leading to a wave of outstanding code generation models and tools. Correspondingly, there are also several benchmarks proposed and widely used for evaluating the performance of automated code generation.

\subsection{LLMs for Code Generation}
% codellama starcoder deepseek metagpt chardev

CodeLlama\cite{codellama} is further trained based on Llama2\cite{llama2}. It is capable of understanding and generating code in various programming languages, including but not limited to Python, Java, JavaScript, etc. CodeLlama not only generates complete code but also provides suggestions and optimization solutions for specific code snippets, greatly assisting developers. During the training of the base model, weights are initialized with an equivalent parameter amount of the Llama2 model, followed by training on a dataset of 500 billion tokens of code. 
% StarCoder\cite{starcoder} is derived from StarCoderBase, which is trained using 10 trillion tokens from The Stack, a vast collection of licensed GitHub repositories with inspection tools and selection exit procedures.
% The DeepSeek-Coder\cite{deepseek} takes into account the often intricate dependency relationships inherent in real-world projects. The model needs to fully consider these dependencies before completing programming tasks. Therefore, to equip DeepSeek-Coder to handle real-world complex projects, the training data is structured to support repository-level comprehension, enhancing the model's understanding of complex projects. This enables the model to utilize cross-file context effectively. 
MetaGPT\cite{metagpt} constructs a multi-agent collaborative framework, employing Standardized Operating Procedures and involving multiple roles such as programmers and product managers to collaborate on project completion. The results generated by agents are not saved in conversational form but in structured output formats such as charts, files, etc. Communication between agents is also conducted through structured files. MetaGPT also implements an iterative development pipeline, optimizing results through multiple rounds of iteration by recording information generated during the development process by different roles. Similarly, ChatDev\cite{chatdev} adopts a multi-agent framework, allocating and assigning different AI agents to various job functions. ChatDev facilitates communication among different role agents, forming a complete software development process where each agent performs its respective tasks while collaborating uniformly.In addition to these models, there are many other excellent models used in the field of code generation\cite{wizardcoder,pangu,pangu2,codegen,codex,AlphaCode,incoder}.

%除了这些模型之外，还有很多优秀的模型被用在代码生成领域。

\subsection{Code Generation Benchmark}
Previously, the vast majority of benchmarks were constructed to evaluate the performance of LLMs in generating standalone functions, with the most representative ones being HumanEval \cite{humaneval} and MBPP \cite{MBPP}. HumanEval comprises 164 manually crafted programming problems, covering aspects such as language comprehension, reasoning, algorithms, and simple mathematics. MBPP consists of 974 short Python function problems primarily designed for novice programmers. 

% As a result, ClassEval was manually crafted, consisting of 100 class-level code generation tasks. However, since these problems do not originate from real-world projects and writing class-level code only requires considering dependencies within the class, ClassEval also cannot effectively reflect the complexity of actual development situations. 

Finding previous benchmarks fail to reflect complex programming scenarios, 
researchers propose CoderEval\cite{codereval}, the first repository-level code generation benchmark, to evaluate the performance of existing LLMs in real-world development by prompting them generate functions selected in actual complex software. CoderEval meticulously selects 230 Python and 230 Java programming tasks from popular real-world open-source projects, evaluating the functional correctness of generated code based on execution. To better simulate real-world development scenarios, DevEval first analyses the distribution of standalone and non-standalone functions in a large number of real-world projects, then constructs a benchmark with a difficulty distribution more in line with real-world scenarios. 
% Considering the extensive cross-file dependencies in real-world software development, researchers proposed CrossCodeEval, a diverse multi-language code completion benchmark that requires a deep understanding of cross-file context to accurately complete code. CrossCodeEval not only evaluates LLMs' ability to use cross-file context but also serves to assess code retrievers' performance in retrieving cross-file context. 



Although the aforementioned works prompt LLMs to generate functions selected from real software projects to evaluate LLM performance in real development scenarios, we recognize a common flaw in all these benchmarks: they ignore the evolution of project repositories. This implies that when we prompt LLMs to generate different functions, the project context provided to LLMs should also consider the evolution of the project. Taking the example of software development processes based on GitHub project management, when writing functions, the project context that programmers can refer to is the entire project repository up to the commit preceding the target functions. Therefore, when prompting LLM to generate target functions, we should first roll back the entire project repository to the state before the target function was committed.
% Based on this, we propose CoderEval2, an evolving-aware repository code generation benchmark.



\subsection{Repository-level Code Generation}
Many technical studies have been proposed to better tackle repository-level code generation tasks\cite{repofusion,docprompting,repocoder}.  
DocPrompting\cite{docprompting} uses natural language (NL) intent to retrieve documents related to the target code, and then sends NL intent and retrieved documents to LLMs. COCOMIC\cite{cocomic} developes a cross-file context finder, which is a static code analysis tool used to retrieve the most related cross-file context. MGD\cite{guiding} leverages IDEs to assist in providing context. When reaching the pre-defined trigger point, IDE is invoked to provide useful suggestions. RLPG\cite{repositorylevel} analyses dependencies potentially existing in the target function, then extract project context that may conducive to generating the target function. RepoCoder\cite{repocoder} first slices the source code files in the Repo to construct a retrieval library, then uses the generated problem as a query, calculates similarity to obtain repo context, and feeds the repo context and problem to the model to generate initial results. After obtaining the initial results, the previous generation results are used as queries for further querying to obtain more context. This process is repeated to continuously optimize the generation results. $A^3$ CodGen\cite{codgen} first constructs a repository knowledge base covering knowledge of third-party libraries and extracts information on mobile and code context. During the code generation process, LLM first generates an initial version of code based on NL intent, then uses NL intent and the initial version of code to retrieve as much foundational knowledge as possible from the knowledge base for the LLM. Finally, local, global, and third-party library information is integrated into the prompt to allow the model to generate the final result.


However, all the mentioned works treat the latest version of the project repository as the context source, falling into the category of evolving-ignored scenarios. Although in RepoCoder, researchers began to take notice of this issue by considering all code after the target function in the corresponding file as "future code", this still falls short of reality and introduces a lack of the context that should originally be present. Therefore, we propose a novel repository-level code generation benchmark, CoderEval2, an evolving-aware pragmatic benchmark, to better simulate real development scenarios for LLMs.


%上面提到的所有这些工作在获取context时都把最新版本的项目仓库当作context source，这显然是不对的。举一个例子，假设程序员在完成函数A的编程时项目正处于version2，此时，对于程序员来说context source就是处于version2的整个项目仓库。随着时间的变迁，现在项目可能更新到了version10，在这个过程中，程序员对项目中的代码做了无数的增加或者修改。而上述工作将函数A作为生成目标的时候本应该提供version2的项目仓库作为context source，但他们缺将version10的项目仓库作为context source，这无疑给LLM提供了一个虚假的编程场景。在RepoCoder中，研究人员开始注意到了这一点，他们将目标函数对应的代码文件中，所有处于目标函数之后的代码都作为"future code"，但是这离真实情况还是差了很远，而且这还会带了本来应该又的context的缺失。归根结底来说，是之前的repotiory-level的code generation benchmark都忽略了项目随着时间的变迁而不断演化这一事实，因此我们的工作主要是为了解决这一痛点，为LLM提供更加真实编程环境。
% All of the mentioned approaches, in obtaining context, have treated the latest version of the project repository as the context source, which is evidently incorrect. To illustrate, suppose a programmer completes the coding for function A while the project is at version 2; at this point, the context source for the programmer is the entire project repository at version 2. However, over time, the project may have progressed to version 10, during which the programmer made numerous additions or modifications to the project code. The aforementioned approaches mistakenly used the project repository at version 10 as the context source when generating function A, providing the LLM with a false programming scenario. 

% In RepoCoder, researchers began to address this issue by considering all code following the target function in the corresponding code file as "future code." However, this approach still falls short of reality and introduces the risk of missing the context that should have been present. Ultimately, the repository-level code generation benchmarks of the past have overlooked the fact that projects evolve over time. Therefore, our work primarily aims to address this pain point by providing LLMs with a more realistic programming environment.

%上面提到的所有这些工作在获取context时都把最新版本的项目仓库当作context source,都属于evolving-ignored的情况，尽管在RepoCoder中，研究人员开始注意到了这一点，他们将目标函数对应的代码文件中，所有处于目标函数之后的代码都作为"future code"，但是这离真实情况还是差了很远，而且这还会带了本来应该有的context的缺失。因此，我们认为十分有必要创建一个evolving-aware的benchamrk来更好地模拟实际开发场景，为LLM提供更加真实编程环境。

==> sections/3_Benchmark.tex <==
\section{CoderEval2 Benchmark}
In this section, we will provide a detailed introduction to CoderEval2 from three perspectives: benchmark overview, benchmark construction pipeline, and benchmark characteristic.
\subsection{Benchmark Overview}

CoderEval2 consists of a total of 400 task instances, comprising 200 Python programming questions and 200 Java programming questions. As illustrated in Figure \ref{figure4}, each task instance is associated with a unique identification number. The "Repo/Owner" field helps identify the GitHub project from which the selected function originates, while the "Version" field indicates the version of the project during the implementation of this function. The process of selecting functions is based on pull requests, so "Base commit" refers to the last commit on the target branch before the pull request is merged, used to restore the project repository to the state that the programmer could reference when implementing the target function. The "Function declaration" of the target function will be provided to the LLM as part of the prompt, along with its corresponding docstring. As depicted in the overview, the brief docstring generally provides a concise summary of the functionality of the target function, while the detailed docstring provides a thorough description of the function's functionality, inputs, and outputs.

\subsection{Benchmark Collection Pipeline}

\begin{figure*}[h]
  \centering
  \includegraphics[width=1\textwidth]{Figures/Collecting-pipeline.pdf}
  \caption{CoderEval2 Construction Pipeline}
  \label{figure3}
\end{figure*}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=1\textwidth]{Figures/Collecting-pipeline1.pdf}
%   \caption{CoderEval2 Construction Pipeline}
%   \label{figure3}
% \end{figure*}

CoderEval2 is an evolving-aware repository-level code generation benchmark designed to simulate the software development process in practice. In real-world development scenarios, numerous large-scale software development activities are conducted based on GitHub project management. When engineers implement new features requested by users, they typically create pull requests to attempt to merge the newly added code into the original project. This additional code undergoes review by repository administrators and, upon confirmation of its accuracy, is merged into the repository. Drawing inspiration from this, we simulate incremental development activities by collecting Pull Requests (PRs) from real projects and selecting the added functions in the PRs as the generation targets for LLMs. AS depicted in Figure \ref{figure3}, the process of collecting the benchmark dataset is similar to \cite{swe}, primarily involving five steps.

%步骤一：project selection。高频使用，高star

\subsubsection{High Quality Projects Selection} To ensure the pragmatism and diversity of CoderEval2, we adopt a comprehensive approach to selecting functions from various open-source projects. For Python, we select high-quality real-world projects from a curated list of the top 5,000 most downloaded PyPI libraries during 2023\footnote{https://hugovk.github.io/top-pypi-packages/}. Subsequently, we meticulously ascertain the corresponding open-source GitHub repositories for each project and verify which packages have licenses permitting free software use. We then proceed to collect pull requests (PRs) for these repositories through the GitHub developer API. For Java, as widely recognized projects typically indicates extensive documentation, structured open-source development guidelines, and functional, well-formatted code, our approach involves searching for the top 200 starred projects on GitHub. Following this, we individually deploy each project and meticulously select repositories that can be successfully deployed, run without errors, and pass all test cases. This methodology ensures that the functions selected for evaluation in CoderEval2 are representative of real-world programming scenarios, encompassing a diverse range of projects and languages.

 
%步骤二 获取PR


\subsubsection{PR Crawling} After completing the high-quality project selection process, we gathers numerous initial PRs from the popular open-source repositories identified in the aforementioned procedure. Each PR is associated with a codebase, representing the state of the repository before the PR was merged. In this step, we obtained 12,039 Pull Requests (PRs) and meticulously recorded metadata pertaining to these PRs for subsequent filtering processes.

%步骤三：Attribute filter  增加了新函数 新增test。被merged
% 

\subsubsection{Attribute Filter} We construct candidate task instances from PRs that meet three criteria. First, the status of the PR be"Merged." A "Merged" status indicates that the code changes associated with the PR were accepted and incorporated into its parent repository. Second, the PR must introduce new functions. These newly added functions are typically intended to develop the software project by adding new features, improvements, or fulfilling general development objectives. Third, the PR must introduce one or more new tests and these tests must cover the selected function. All these attributes are aimed at ensuring that the subsequently selected functions are of high quality, having undergone rigorous review and being covered by the project's testing framework.



%步骤四：execution filter


\subsubsection{Execution-based Filter} In this step, we perform validation based on execution for the PRs filtered in attribute filter step. For each task instance, we first determine the version of the project corresponding to the PR, then manually identify the required dependency environment for running the project at that version. For example, for a Python task instance, we should confirm the required Python version and the types and versions of third-party libraries it depends on. After obtaining this dependency environment information, we create a virtual execution environment for each version of the project. During this step, task instances that can not install the dependency environment properly are filtered out. After creating the execution environment, we execute the project's testing framework in the corresponding environment.

To ensure that the project's test suite covers the newly added functions, we further process the PR's patch file. Generally speaking, source code in a project can generally be divided into two categories: production code and test code. Similarly, we divide the PR's patch into production patch and test patch. For each candidate task, we apply the PR’s test content and log the associated test results before and after applying the PR’s other content. We filter out task instances without at least one test where its status changes from a fail to pass, which indicates the newly added functions are definitely covered by the test suite. After filtering out instances without a fail-to-pass transition, we obtain 400 PRs.


%步骤五：human annotation

\subsubsection{Human Annotation} We recruit six experienced software developers to manually craft docstrings for each task instance. Firstly, to provide detailed requirement descriptions for the Language Model (LLM) to better generate functions, we requested developers to write a comprehensive comment for each task instance, including details of each input and output parameter. After the programmers completed writing the docstrings, we conducted a cross-check review, requiring each task instance to be verified and confirmed by two engineers to ensure accuracy. Otherwise, the docstring would be rewritten, and the cross-check process would be repeated. Secondly, during the data collection process, we observed that developers tend to write relatively simple docstrings in actual projects, often providing a basic description of the function's functionality. Therefore, to simulate the use of LLM in real-world development scenarios, we asked software developers to generate a brief docstring for each task instance once again. Similarly, we conducted cross-check reviews for these docstrings.

Finally, to better analyze the performance of LLM on CoderEval2 from multiple perspectives, we further categorized all task instances in CoderEval2 based on dependency levels, resulting in three categories: stanalone, intra-class, and inter-class.

%这一段用来静态分析：四个依赖级别的百分比
%Among the retained functions, 862 are standalone, and 1,984 are non-standalone. We follow the distribution of program types in 500 practical projects to construct DevEval, ensuring the data size is maximized. Retaining all 1,984 (73.8%) non-standalone functions, we randomly sample 706 (26.2%) standalone functions, resulting in the DevEval with 2,690 samples.

%这两部分也可以考虑合并起来
% \subsection{Dataset Inspection}

%1. 划分的四种依赖level的数据(这里来两个饼状图)。注明一下intra-file是必须external-class / outside-class，不备注的话intra-file其实是包括intra-class,这里可以看看DevEval，结果跟我们想的相反，如果感觉有歧义的话，就把intra-class直接去掉，就standalone/intra-file/cross-file
%java依赖一般都比较深，因为一般都是一个文件一个class，class之间交互
%python:
% standalnoe:    50     0.2336448598130841
% intra-class:   61     0.2850467289719626
% intra-file:    43     0.20093457943925233
% cross-file     60     0.2803738317757009
%interclass
%java
% standalnoe:    37     0.17535545023696683
% intra-class:   61     0.2890995260663507
% intra-file:    4      0.018957345971563982
% cross-file     109    0.5165876777251185
%要不就直接划分成standalone 和 non-standalone，然后说这是一个足够challenge

%2. 各种长度的对比？ （表格）

%2.1 跟HuamnEval比平均函数长度
%python

%java




\subsection{Benchmark Characteristic}

%一：evolving-aware


\subsubsection{\textbf{Evolving-aware benchmark. }} We identify a crucial issue that previous research has neglected: the development of a project is an evolving process, leading to the context accessible to programmers evolving across different stages of development. Previous studies have overlooked this temporal dimension, resulting in large models being fed with code that had not yet been implemented in the project when certain functions were developed. Consequently, it also misses some context that should have been present but might have been deleted or updated during the project's evolution. This undoubtedly leads to the model facing an unrealistic development scenario. As a result, the performance of large language models in real-world software development tasks remains unknown. Therefore, we are committed to refining CoderEval2 into a benchmark that better simulates real-world software code development scenarios, aiming to more accurately reflect the true performance of LLMs applied to pragmatic development tasks.

%二 严格的数据筛选流程

\subsubsection{\textbf{Strict data filtering process.}} First, we ensure that the selected projects are of high quality, because high-quality projects generally have excellent maintenance, comprehensive testing frameworks, and good coding styles, which make our benchmark more representative.. For Python, we choose the projects with the highest download count in PyPI. For Java, we select projects from the top 200 projects on GitHub based on the number of stars, with an average of around 24k stars.  Previous benchmarks have ensured the functionality of target functions by writing unit tests for each function separately. However, we believe that in a project with complex dependencies, adding a new function may have certain impacts on other parts of the project. Relying solely on unit tests for the target function is insufficient to ensure that the project can still function properly and pass the project's test framework after inserting the function. Therefore, in this work, we directly run the project's test framework to ensure the correctness of the target function's functionality while ensuring that inserting the target function does not have a negative impact on other parts of the project. Of course, to ensure that the test framework covers the target function, during the function selection process, we verify that our selected functions are covered by the project's test framework through execution-based validation. In other words, a "fail-to-pass" test result implies that the test is set up for the target function and the target function has passed the test.

%四：human annotation / 划分了dependent level / 

\subsubsection{\textbf{Human annotation.} }
During the dataset construction process, we observed variations in annotation styles among these high-quality projects, generally categorized as detailed and brief. Detailed annotations typically provide comprehensive descriptions of a function's functionality, elucidate input and output parameter types, and annotate potential error scenarios. Conversely, brief annotations succinctly outline the function's functionality in a few sentences. To enhance the diversity of our benchmark and better align with real-world development scenarios, we manually crafted two versions of annotations for each function: detailed and brief. This provides users with more options for subsequent usage.

Furthermore, to better explore the performance of LLMs in practical development, we categorized the selected functions based on their dependency levels, including standalone, intra-class, and inter-class. Standalone functions can be implemented without relying on other functions within the project. Intra-class functions typically require dependencies on other functions within the same class, usually located in the same file. Inter-class functions imply more complex dependencies, with most of the dependent functions located in other files of the project. Manual categorization of dependency levels aids in analyzing the performance of LLMs in generating functions of varying complexity, facilitating researchers in improving the application of LLMs in practical development scenarios based on different contexts. Moreover, as indicated in the table \ref{dependent level}, the majority of our benchmark comprises functions with deep dependency levels. This suggests that our benchmark presents a sufficiently challenging scenario.


\begin{table}[t]
\centering
\caption{Dependency Level In CoderEval2}
\label{dependent level}
\renewcommand{\arraystretch}{1.5} 
\begin{tabular}{ccc}
\hline
Dependency Level& CoderEval2-Python &CoderEval2-Java\\
\hline
Standalone & 50(23.4\%) &37(17.5\%)\\
Intra-class& 61(28.5\%) &61(28.9\%)\\
Inter-class &103(48.1\%) & 113(53.6\%) \\
\hline
\end{tabular}
\end{table}


%五。 还标注了code创建的时间 / 可以参考一下SWE-bench的continually updatable：collection process can be easily applied to any Python repository on GitHub



\subsubsection{\textbf{A pipeline that can effectively prevent data leakage.}} 
Due to the prevalent adoption of pre-training mechanisms in training large models, which necessitate extensive datasets and powerful computational resources, the training process aims to enable models to learn universal features and knowledge for subsequent fine-tuning or transfer learning tasks. To achieve better performance during the pre-training phase, model trainers typically collect available code from GitHub for model training. This practice has led to the possibility of data leakage, where the data selected by previous benchmarks may inadvertently be included in the pre-training data. Our established data collection process effectively mitigates this concern. We have developed a fully automated data collection pipeline, as depicted in Figure 4, which periodically updates our dataset. This ensures that the target functions we have selected do not appear in the model's training set.

\begin{figure}[t]
  \centering
  \includegraphics[width=0.5\textwidth]{Figures/TaskInstance.pdf}
  \caption{Task Instance Overview}
  \label{figure4}
\end{figure}

==> sections/4_Experiments.tex <==
\section{Experiments SETUP}

\begin{table*}[t]
    \centering
    \caption{RQ1: How does LLM perform under the evolving-aware and evolving-ignored conditions?}
    \label{RQ1}
    \renewcommand{\arraystretch}{1.5} 
    \scalebox{1}{\begin{tabular}{c|cc|cc}
    \hline
        \multirow{2}{*}{Model}  & \multicolumn{2}{c}{Python} &  \multicolumn{2}{c}{Java}\\ 
        \cmidrule(lr){2-3} \cmidrule(lr){4-5}
       ~ & Evolving-ignored & Evolving-aware &Evolving-ignored & Evolving-aware\\
       \hline
       CodeLlama-7b  &58&\cellcolor{blue!5}44 ($\downarrow 24.1\%$)&17&\cellcolor{blue!5}12 ($\downarrow 29.4\%$)\\
       CodeLlama-13b &61&\cellcolor{blue!5}46 ($\downarrow 24.6\%$)&19&\cellcolor{blue!5}14 ($\downarrow 26.3\%$)\\ 
       CodeLlama-34b &63&\cellcolor{blue!5}48 ($\downarrow 23.8\%$)&29&\cellcolor{blue!5}20 ($\downarrow 31.0\%$)\\
       DeepSeek Coder-6.7b &60&\cellcolor{blue!5}46 ($\downarrow 23.3\%$)&26&\cellcolor{blue!5}18 ($\downarrow 30.8\%$)\\
       DeepSeek Coder-33b &62&\cellcolor{blue!5}50 ($\downarrow 19.4\%$)&31&\cellcolor{blue!5}23( $\downarrow 25.8\%$)\\
       GPT-3.5-turbo &65&\cellcolor{blue!5}51 ($\downarrow 21.5\%$)&36&\cellcolor{blue!5}26 ($\downarrow 27.8\%$)\\
       GPT-4&69&\cellcolor{blue!5}53 ($\downarrow 23.2\%$)&41&\cellcolor{blue!5}29 ($\downarrow 29.3\%$)\\\hline
    \end{tabular}}
\end{table*}

%尽量调整成单栏
\begin{table*}[t]
    \centering
    \caption{Overlapping: condition1: EA pass but EI fail; condition2: EA pass and EI pass; condition3: EA fail but EI pass}
    \label{RQ1}
    \renewcommand{\arraystretch}{1.5} 
    \scalebox{1}{\begin{tabular}{c|ccc|ccc}
    \hline
        \multirow{2}{*}{Model}  & \multicolumn{3}{c}{Python} &  \multicolumn{3}{c}{Java}\\ 
        \cmidrule(lr){2-4} \cmidrule(lr){5-7}
       ~ & condition1 & condition2 &condition3 & condition1 & condition2 &condition3\\
       \hline
       CodeLlama-7b  &7&37&21  &3&9&8\\
       CodeLlama-13b &4&42&19  &3&11&8\\ 
       CodeLlama-34b &2&46&17  &6&14&15\\
       Deepseek-Coder-6.7b &4&42&18  &7&11&15\\
       Deepseek-Coder-33b &4&46&16   &5&18&13\\
       GPT-3.5-turbo &2&49&16   &10&16&20\\
       GPT-4         &0&53&15       &4&25&16\\\hline
    \end{tabular}}
\end{table*}





In this section, we will delve into the experimental details, primarily concentrating on three key aspects. Firstly, we will introduce the base Large Language Models (LLMs) utilized in the experiments and elucidate the rationale behind our selection of these models. Secondly, we will outline the research questions that the experiments aim to address. Lastly, we will provide a comprehensive description of the experimental setup employed in our study. Through these detailed explanations, we aim to offer a thorough understanding of the methodologies and motivations underpinning our experimental approach.

\subsection{Base LLMS}
%介绍模型 codellama(7b,13b, 34b) deepseek(6.7b,33b) gpt-3.5-turbo  gpt4


We begin by categorizing the available large language models (LLMs) for code generation tasks into two distinct groups: open-source and closed-source LLMs. For open-source LLMs, our initial selection includes the Codellama series, encompassing the 7b-version, 13b-version, and 34b-version. Renowned for their widespread acclaim within the field, the Codellama series of LLMs are considered highly representative and have garnered significant attention. Additionally, we have chosen the Deepseek Coder series of LLMs, featuring the 6.7b-version and 33b-version. These models have consistently demonstrated state-of-the-art performance in coding proficiency across various programming languages and have excelled in diverse benchmark tests within the domain of open-source code models. On the other hand, for closed-source LLMs, we have selected commonly used commercial models, specifically gpt-3.5-turbo and gpt4. The choice of these models is attributed to their widespread usage and recognition, with gpt4 being acknowledged as one of the most powerful LLMs available in the market. 

Through this categorization and selection process, we aim to encompass a diverse range of LLMs representative of both open-source and closed-source domains, thereby facilitating comprehensive experimentation and analysis in our study.

\subsection{Research questions}
Our experiment intends to answer the following research questions:
%1. LLM在evolving-awre和evolving-ignored这两种不同的前提下表现如何？
%2. LLM在生成不同依赖level的函数时表现如何？
%3. 在evolving-ignored的情况下，LLM面对的代码生成场景是如何慢慢偏离现实的？
%4. LLM在不同注释风格下表现如何？
\begin{itemize}
    \item RQ1: How does LLM perform under the evolving-aware and evolving-ignored conditions?
    % \item RQ2: How does LLM perform when generating functions with different levels of dependency?
    \item RQ2: How does the code generation scenario faced by LLM gradually deviate from reality, in the case of "evolving-ignored"?
    \item RQ3: How does LLM perform under different commenting styles?
\end{itemize}





\subsection{Experiments Settings}
%RAG / metric
\subsubsection{Retrieval-Augmented Generation}


Due to the intricate dependency relationships commonly found in modern software source code, developers often need to reference the context within a project to clarify these dependencies. Large language models (LLMs) are no exception to this requirement. However, given the enormity of code repositories, it is practically infeasible to include all files from the entire repository in the prompt. Therefore, we adopt a strategy of leveraging similarity retrieval to identify potentially beneficial context from the repository for generating target code.

For each task instance, we first restore the project repository to the state before the target code was committed. Then, we proceed to construct a corresponding context retrieval database by partitioning the code files from the repository into a collection of code snippets. Subsequently, we utilize the docstring of the target code as the query for retrieval and compute the similarity between this query and all code snippets in the context retrieval database. Finally, we select project contexts with higher similarity scores based on the ranking of these similarity scores.

\subsubsection{Evaluation}


We assess the code generated by Large Language Models (LLMs) based on its functional correctness. Our evaluation process involves replacing the target code in the repository with the code generated by the LLM and subsequently executing the entire project's test suite.

In the case of Python repositories, the majority of selected projects utilize pytest to construct their testing frameworks. Therefore, to ensure that the code generated by LLMs aligns with the project's requirements, we directly execute the pre-existing testing frameworks within the projects. Only when all test cases pass with a "PASSED" status do we consider the generated function to be correct. Similarly, for Java projects, we focus on repositories based on either Maven or Gradle, both of which feature mature testing frameworks. After replacing the code generated by LLMs, we require all test cases to pass with a "PASSED" status to validate the generated results. The overall performance of the LLMs is reflected in the pass rate of the tests, providing a quantitative measure of their functional correctness. 

This rigorous evaluation process ensures that the code generated by LLMs meets the functional requirements of the projects and accurately reflects their intended functionality.



==> sections/5_Results.tex <==
\section{EXPERIMENTAL RESULTS}

\begin{table*}[h]
    \centering
    \caption{RQ2 dependent level}
    \label{RQ2}
    \renewcommand{\arraystretch}{1.5} 
    \scalebox{1}{\begin{tabular}{c|c|cc|cc}
    \hline
        \multirow{2}{*}{Dependent-Lvel} &\multirow{2}{*}{Model}  & \multicolumn{2}{c}{Python} &  \multicolumn{2}{c}{Java}\\ 
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
       ~& & Evolving-ignored & Evolving-aware  & Evolving-ignored & Evolving-aware \\\hline
       % \multirow{7}{*}{Standalone} 
       %   &CodeLlama-7b &10&7 ($\downarrow 30.0\%$)&3&4 ($\uparrow 33.3\%$)\\
       % ~ &CodeLlama-13b &11&8 ($\downarrow 27.3\%$)&3&4 ($\uparrow 33.3\%$)\\
       % ~ &CodeLlama-34b &11&8 ($\downarrow 27.3\%$)&6&3 ($\downarrow 50.0\%$)\\
       % ~ &Deepseek-Coder-6.7b  &11&8 ($\downarrow 27.3\%$)&4&2 ($\downarrow 50.0\%$)\\
       % ~ &Deepseek-Coder-33b &10&7 ($\downarrow 30.0\%$)&8&5 ($\downarrow 37.5\%$)\\
       % ~ &GPT-3.5-turbo   &11&9 ($\downarrow 18.2\%$)&8&6 ($\downarrow 25.0\%$)\\
       % ~ &GPT-4    &13&9 ($\downarrow 30.8\%$)&10&7 ($\downarrow 30.0\%$)\\\hline
       \multirow{7}{*}{Intra-Class} 
         &CodeLlama-7b &20&19 ($\downarrow 5.0\%$)&1&1\\
       ~ &CodeLlama-13b &18&17 ($\downarrow 5.6\%$)&3&2 ($\downarrow 33.3\%$)\\
       ~ &CodeLlama-34b &21&17 ($\downarrow 19.0\%$)&5&4 ($\downarrow 20.0\%$)\\
       ~ &Deepseek-Coder-6.7b  &21&17 ($\downarrow 19.0\%$)&3&2 ($\downarrow 33.3\%$)\\
       ~ &Deepseek-Coder-33b &23&21 ($\downarrow 8.7\%$)&2&2\\
       ~ &GPT-3.5-turbo   &22&18 ($\downarrow 18.2\%$)&3&3\\
       ~ &GPT-4    &23&20 ($\downarrow 13.0\%$)&5&3 ($\downarrow 40.0\%$)\\\hline
       \multirow{7}{*}{Inter-Class} 
         &CodeLlama-7b &28&18 ($\downarrow 35.7\%$)&12&6 ($\downarrow 50.0\%$)\\
       ~ &CodeLlama-13b &32&21 ($\downarrow 34.4\%$)&12&7 ($\downarrow 41.7\%$)\\
       ~ &CodeLlama-34b &31&23 ($\downarrow 25.8\%$)&17&12 ($\downarrow 29.4\%$)\\
       ~ &Deepseek-Coder-6.7b  &28&21 ($\downarrow 25.0\%$)&18&13 ($\downarrow 27.8\%$)\\
       ~ &Deepseek-Coder-33b &29&22 ($\downarrow 24.1\%$)&20&15 ($\downarrow 25\%$)\\
       ~ &GPT-3.5-turbo   &32&24 ($\downarrow 25.0\%$)&24&16 ($\downarrow 33.3\%$)\\
       ~ &GPT-4    &33&24 ($\downarrow 27.3\%$)&25&18 ($\downarrow 28.0\%$)\\\hline
       
    \end{tabular}}
\end{table*}

\subsection{ RQ1: How does LLM perform under the evolving-aware and evolving-ignored conditions?}


\subsubsection{Overall effectiveness}


Table \ref{RQ1} presents the performance of seven mainstream models on CoderEval2. We conducted two experimental settings: Evolving-ignored (where the context source is the latest version of the project repository) and Evolving-aware (where the context source is the project repository before the target function is committed). From the experimental results, it can be observed that on CoderEval2-Python and CoderEval2-Java, there is a significant decrease in performance under the Evolving-aware setting. This indicates that the aforementioned Evolving-ignored scenario leads to a deviation in the model's performance from its performance in actual development scenarios. The models exhibit false performance after referencing a large amount of context that should not exist.

\subsubsection{Overlap}


In Figure \ref{figure1}, two instances occurring under the evolving-ignored scenario are illustrated. The first scenario introduces an "extra" context that should not exist, thereby inflating the model's performance. However, in the second scenario, certain context that should exist disappears as the project evolves. Generally, the disappearance of such context leads to a decrease in model performance. However, from the results in Table \ref{RQ1}, it appears that the model's performance only exhibits an inflated trend. Does this mean that the second scenario depicted in Figure 1 did not occur? With this question in mind, we investigated the overlap between task instances that the models were able to complete under these two settings.

In Table \ref{overlap}, "condition1" refers to the number of instances that passed under the Evolving-aware (EA) setting but failed under the Evolving-ignored (EI) setting. "Condition2" denotes the number of instances that passed under both settings, while "condition3" represents instances that failed under EA but passed under EI. We found that both scenarios depicted in Figure 1 were indeed at play. Condition1 primarily arises due to the absence of necessary context. From the experimental results, it is evident that except for GPT-4 in CoderEval2-Python, which had a value of 0 for condition1, all other models exhibited deviations from reality caused by the absence of necessary context in a certain quantity. However, the primary influencing factor remains the evolution of the project, which introduces more extraneous context that should not exist.
\subsubsection{Dependent level}


During repository-level code generation, it is crucial to reference project context to comprehensively understand the intricate dependencies between functions. Instances in the CoderEval2 benchmark can be categorized into two types based on dependency levels: standalone and non-standalone (intra-class and inter-class). When generating non-standalone functions, it is necessary to reference the functions upon which these models depend to understand their parameter interfaces and complete the function invocation process. Because evolving-ignored directly affects the available context source for the models, we investigated the performance of LLM in generating these functions with complex dependencies under two scenarios: context-ignored and context-aware.

As shown in Table \ref{dependent level}, under the evolving-aware scenario, the accuracy of LLM in generating both intra-class and inter-class functions has noticeably declined. The decline is more pronounced for inter-class functions, as these functions typically require cross-file context, which is often more scattered. As the project evolves, its various parts tend to become more comprehensive. Therefore, under the evolving-ignored setting, the models can reference an increasing amount of context. Consequently, when the evolving-aware setting loses access to these contexts, the model's performance significantly deteriorates.


\begin{tcolorbox}[title = {Findings}] 
Through experimentation, we observed an inflated trend in LLM's performance under the Evolving-ignored setting. Upon further investigation, we discovered that both the presence of too much extraneous context and the disappearance of context that should exist have significantly affected the model's performance.
\end{tcolorbox}

% \subsection{RQ2: How does LLM perform when generating functions with different levels of dependency?}



\subsection{RQ2: How does the evolving-ignored code generation scenario gradually deviate from reality?}

To further illustrate the impact of the evolving-ignored setting on the performance of LLMs as projects evolve, additional experiments were conducted. Typically, a model's version number consists of three digits in the format "0.0.0," where the first digit represents the major version, the second digit represents the minor version, and the last digit represents the patch version. To simulate the evolution process of a project, in Figure \ref{RQ3}, we start with evo0 (evolving-aware) and increment the minor version number by one each time. If there are no more minor versions under that major version, the major version is incremented. We do not update the patch version because patch versions are generally numerous and entail minimal changes to the project. As depicted in Figure \ref{RQ3}, with the evolution of the project, the model's generated results gradually deviate from reality. However, the artificial improvement in model performance induced by the evolving-ignored setting does not exhibit a linear increase but rather a curve indicating an upward trend. This is primarily due to the fact that not every version update provides contextual information that assists in generating the target function. Some irrelevant contexts introduce noise, resulting in a decline in the final results.

% 在evolving-ignored的设定中，随着项目的演化，LLM面临的代码生成场景逐渐偏离了实际开发场景，模型的表现也成曲折变化的趋势偏离真实表现。
\begin{tcolorbox}[title = {Findings}] 
In the evolving-ignored setting, as the project evolves, the code generation scenarios encountered by LLMs gradually diverge from actual development scenarios, and the model's performance exhibits a trend of convoluted changes departing from real performance.
\end{tcolorbox}
\subsection{RQ3: How does LLM perform under different commenting styles?}










% standalone下降的概率更高的一些解释：
% 1. （首先解释这些函数解决起来难度较大导致EI情况下基数较少）从repo中选择出来的standalone本身难度就高, standalone函数的平均代码函数为33.78，远远超过HumanEval的平均7.8行。而且因为函数是从PyPI的项目中选择的，包含了一些Usage Example function，所以难度也会比较大。从实验结果可以看出来，模型能正确生成的standalone的函数个数也不多。正因为基数较少，零星地几个个数的减少就会带来大较大的比率。

%要不能不能就只看intra-class和inter-class，就看这些需要依赖的函数的情况，这样下降趋势就很明显了



%data leakage
% ----------------------------------------------------
% 时间              before23     after23 
% GPT4             61 / 170      7 / 44
% GPT3.5           56 / 170      9 / 44
% CodeLlama34b     55 / 170      10/44
% CodeLlama13b     55 / 170      8 / 44
% CodeLlama7b      54 / 170      8 / 44

%从比例上来讲没办法说明 没有数据泄露，因为before23的确实成功率更高，应该是数据收集的时候before23的有部分是偏向于简单的？
%但是对于数据泄露这个话题，在CoderEval和DevEval中都没有去详细讨论，像CoderEVal就认为自己重写了docstring就可以避免data leakage

% 依赖-python (GPT4)
% ----------------------------------------------------
%python
% standalnoe:    50     0.2336448598130841
% intra-class:   61     0.2850467289719626
% intra-file:    43     0.20093457943925233
% cross-file     60     0.2803738317757009
%java
% standalnoe:    37     0.17535545023696683
% intra-class:   61     0.2890995260663507
% intra-file:    4      0.018957345971563982
% cross-file     109    0.5165876777251185


%evolving-ignored
% standalnoe:   13 0.26
% intra-class:  23 0.3770491803278688
% intra-file:   13 0.3023255813953488
% cross-file    19 0.316666666666 66665

%evolving-aware
% standalnoe:   9  0.18
% intra-class: 20  0.32786885245901637
% intra-file:   8  0.18604651162790697
% cross-file   16  0.26666666666666666


%noise导致standalone下降，给case study 不相关的context
% \begin{table*}[h]
%     \centering
%     \caption{RQ2: How does LLM perform when generating functions with different levels of dependency?}
%     \label{RQ2}
%     \renewcommand{\arraystretch}{1.5} 
%     \scalebox{1}{\begin{tabular}{c|c|cc|cc}
%     \hline
%        \multirow{2}{*}{Dependent-Level} & \multirow{2}{*}{Model}  & \multicolumn{2}{c}{Python} &  \multicolumn{2}{c}{Java}\\ 
%         \cmidrule(lr){3-4} \cmidrule(lr){5-6}
%       & ~ & Evolving-ignored & Evolving-aware &Evolving-ignored & Evolving-aware\\ \hline
%       \multirow{7}{*}{Standalone} & & & & &\\
%        & & & & &\\
%        & & & & &\\
%        & & & & &\\
%        & & & & &\\
%        & & & & &\\
%        & & & & &\\ \hline
       
   
%     \end{tabular}}
% \end{table*}
% 因为evolving-ignored存在着两种情况，不一定说evolving-aware就会带来效果的下降（参考那两个例子）
% 以GPT-4在Java数据集上的表现为例：
% evolving-aware：26
% evolving-ignored： 36
%这两种情况下都是pass的instance ： 21
% evolving-aware中pass但是evolving-ignored中failed：5
% evolving-aware中failed但是evolving-ignored中pass：15
%when it fails RQ1的分析分成总体的探究和细节的探究
%基于这些结果，先前的“防止作弊”说法可以换成 还原更真实的开发场景

% 共有的元素: {'e7f6c011776e', 'a88a7902cb4e', '2858dcd1057d', 'e0f05da93a0f', '8d27ba37c5d8', 'eeca91fd439b', '80c3cd40fa35', '48449a14a4ff', '968076be2e38', 'd6f0c71ef0c8', '811786ad1ae7', 'eb624dbe56eb', '96061e92f58e', 'd4ee9f58e586', 'a512db2741cd', '31489056e091', 'ef2d127de37b', '2c624232cdd2', '16badfc6202c', '73d3f1ba0625', '922c7954216c'}
% 21
% before_success 有但 after_success 没有的元素: {'98010bd9270f', '6e4001871c0c', '1dfacb2ea5a0', 'd6a403173361', '5ef6fdf32513'}
% 5
% after_success 有但 before_success 没有的元素: {'031b4af5197e', 'd4735e3a265e', '69f59c273b6e', '8527a891e224', '5ec1a0c99d42', '5cf4e26bd3d8', '7902699be42c', 'ff5a1ae012af', '3fdba35f04dc', 'a21855da08cb', '2abaca4911e6', 'b8aed072d294', '02d20bbd7e39', '39fa9ec190ee', '3ada92f28b4c'}
% 15


% \begin{figure}[h]
%   \centering
%   \includegraphics[width=0.5\textwidth]{Figures/overlapping.pdf}
%   \caption{Evolving-ignored situation one: too much "extra" context}
%   \label{overlapping}
% \end{figure}

% \begin{figure*}[h]
%   \centering
%   \includegraphics[width=0.8\textwidth]{Figures/RQ2.pdf}
%   \caption{RQ2}
%   \label{RQ2}
% \end{figure*}
 


 



\begin{figure*}[h]
  \centering
  \includegraphics[width=0.9\textwidth]{Figures/RQ3.pdf}
  \caption{RQ3: How does the code generation scenario faced by LLM gradually deviate from reality, in the case of "evolving-ignored"?}
  \label{RQ3}
\end{figure*}

\begin{table*}[t]
    \centering
    \caption{RQ3: How does LLM perform under different commenting
styles? }
    \label{RQ3}
    \renewcommand{\arraystretch}{1.5} 
    \scalebox{1}{\begin{tabular}{c|c|cc|cc}
    \hline
        \multirow{2}{*}{Model} & \multirow{2}{*}{docstring} & \multicolumn{2}{c}{Python} &  \multicolumn{2}{c}{Java}\\ 
        \cmidrule(lr){3-4} \cmidrule(lr){5-6}
       ~ & & Evolving-ignored & Evolving-aware &Evolving-ignored & Evolving-aware\\ \hline
        \multirow{2}{*}{CodeLlama-7b} 
        &Detailed &58&44&17&12\\
        &Brief &57&44&&  \\\hline
        \multirow{2}{*}{CodeLlama-13b} 
        &Detailed &61&46&19&14\\
        &Brief &60&45&&  \\\hline
        \multirow{2}{*}{CodeLlama-34b} 
        &Detailed &63&48&29&20\\
        &Brief &62&49&&  \\\hline
        \multirow{2}{*}{Deepseek-Coder-6.7b} 
        &Detailed &60&46&26&18\\
        &Brief &60&46&&  \\\hline
        \multirow{2}{*}{Deepseek-Coder-33b} 
        &Detailed &62&50&31&23\\
        &Brief &48&62&&  \\\hline
        \multirow{2}{*}{GPT-3.5-turbo} 
        &Detailed &65&51&36&26\\
        &Brief &&&&  \\\hline
        \multirow{2}{*}{GPT-4} 
        &Detailed &69&53&41&29\\
        &Brief &&&&  \\\hline
     
    \end{tabular}}
\end{table*}

==> sections/6_RealtedWork.tex <==
\section{Related Work}


CoderEval\cite{codereval} is the first benchmark to propose repository-level code generation. It categorizes data into six types based on dependency types: functions that do not require external code, functions that only require standard library imports, functions that require third-party library imports, functions that require code from within the class but outside the function, functions that require code from outside the class but within the file, and functions that require code from other files. The dataset contains 230 samples from 43 Python projects and 230 samples from 10 Java projects.

DevEval\cite{deveval}, compared to CodeEval, collected data from more repositories (119) and included a richer set of programming tasks (2690). It also ensured that the distribution of programming tasks (with or without dependencies) matched the distribution of real repositories. Compared to CodeEval, each sample in DevEval also included more comprehensive information.

Existing LLM code generation benchmarks focus on function-level or statement-level (standalone code), lacking evaluation of code generation tasks in complex scenarios. Thus, ClassEval\cite{classeval} focuses on evaluating class-level code generation tasks. ClassEval is manually constructed and comprises 100 class-level Python code generation tasks.

Taking HumanEval\cite{humaneval} as an example, previous benchmarks included NL intent and function signature in the constructed prompts. However, because class-level code generation involves dependencies and method interfaces, prompts need to contain more information. The authors categorized this information into two types: (1) class-level information, including import statements, class name, class description, and class constructor; (2) method-level information, including method signature, functional description, parameter/return description, and example input/outputs.



Repocoder\cite{repocoder} proposed RepoEval, which consists of the latest and high-quality real-world repositories covering scenarios such as line completion, API invocation, and function body completion. CROSSCODEEVAL\cite{crosscodeeval} can be used to evaluate a model's ability to complete code using cross-file context information. In the examples of CROSSCODEEVAL, the statements to be completed must include at least one API defined in other files. XCODEEVAL\cite{xcodeeval} is the largest execution-based multi-language multi-task benchmark to date, containing approximately 7.5k different tasks, covering up to 11 execution-based programming languages with parallelism. It includes seven tasks: code comprehension, code generation, code translation, and code search.

Currently, most benchmarks for LLM code generation provide simple functions, mostly targeting general functions rather than specific domains, thus limiting practicality. However, BioCoder\cite{biocoder}, a benchmark for bioinformatics code generation, has been introduced. BioCoder carefully selected 28 high-quality projects related to bioinformatics, then parsed these repos to generate ASTs and obtain relevant data. A custom code context was written for each filtered function, including necessary imports, cross-file dependencies, and some test cases.

% AN EXECUTION-BASED LARGE SCALE MULTILINGUAL MULTITASK BENCHMARK FOR CODE UNDERSTANDING, GENERATION, TRANSLATION AND RETRIEVAL。

==> sections/7_ThreatsToValidity.tex <==
% \section{Threats to validity}

% \subsubsection{Base LLM selection. }
% %在选择base LLM时，由于计算资源有限，我们只对部分比较受欢迎的LLM进行了评测，没有覆盖到其他优秀的大模型（StarCoder，Claude系列，WizardCoder等），这在一定程度上可能无法完全反映出当今LLM在实际开发工作中的真实实践表现。
% \subsubsection{Data Leakage.}
% %这里需要一点实验。
% \subsubsection{Classification of different levels of dependence}
% %在对所选函数的依赖等级进行划分时，可能因为统计原因，没办法完成收集到所有的第三方库信息，因此在依赖等级划分部分可能会存在一点偏差。





==> sections/8_Conclusion.tex <==
\section{Conclusion}


In this paper, we begin by highlighting a previously overlooked aspect by existing repository-level code generation benchmarks: the evolution of project development over time. We observe that as projects evolve, the available project contexts for reference also undergo changes. Building upon this observation, we introduce CoderEval2, an evolving-aware repository code generation benchmark. CoderEval2 is designed to more realistically simulate the scenarios encountered in actual development settings by considering the temporal evolution of projects. Through CoderEval2, we experimentally evaluate the performance of various large language models, including Codellama (7b, 13b, 33b), Deepseek Coder (6.7b, 33b), gpt-3.5-turbo, and gpt4, when applied in practical development settings. By incorporating temporal considerations into the benchmark, CoderEval2 provides a more comprehensive assessment of model performance, taking into account the dynamic nature of project development.

We believe that CoderEval2 will offer valuable insights for the future development of large-scale code models, enabling researchers and practitioners to better understand and improve the effectiveness of these models in real-world development scenarios.
